Private, Efficient and Scalable Kernel Learning for Medical Image Analysis

Medical imaging is key in modern medicine. From magnetic resonance imaging (MRI) to microscopic imaging for blood cell detection, diagnostic medical imaging reveals vital insights into patient health. To predict diseases or provide individualized therapies, machine learning techniques like kernel methods have been widely used. Nevertheless, there are multiple challenges for implementing kernel methods. Medical image data often originates from various hospitals and cannot be combined due to privacy concerns, and the high dimensionality of image data presents another significant obstacle. While randomised encoding offers a promising direction, existing methods often struggle with a trade-off between accuracy and efficiency. Addressing the need for efficient privacy-preserving methods on distributed image data, we introduce OKRA (Orthonormal K-fRAmes), a novel randomized encoding-based approach for kernel-based machine learning. This technique, tailored for widely used kernel functions, significantly enhances scalability and speed compared to current state-of-the-art solutions. Through experiments conducted on various clinical image datasets, we evaluated model quality, computational performance, and resource overhead. Additionally, our method outperforms comparable approaches

==> 0-abstract.tex <==
\begin{abstract}

%This approach is particularly crucial for the identification and management of rare diseases, where the scarcity of available data poses unique challenges. 

%This paper discusses the importance of ML in interpreting medical imaging for rare diseases and explores innovative solutions to overcome the challenges posed by small datasets with high-dimensional data. 

%This issue is further compounded in the context of clinical image data, such as X-rays and MRI scans. These data types are not only sensitive but also inherently high-dimensional, making their processing and analysis a complex task. 


%Today's healthcare system is undergoing a paradigm shift, moving away from a 'one-size-fits-all' approach towards medical treatments based on individual patient characteristics. Machine Leaning has the potential to support this paradigm shift with the prediction of disease progression and selection of targeted therapies. Medical images, such as MRI, CT scans, and X-rays can reveal critical insights into patient health. However, this data is sensitive, high-dimensional, and typically distributed across different data holders. It's even more difficult for rare diseases, where limited availability of data hinders the development of robust models. The key challenge lies in performing privacy-preserving machine learning on small, distributed datasets with high-dimensional data.

%To address this problem, we propose OKRA (Orthonormal K-fRAmes), a one-shot federated learning algorithm designed for privacy-preserving kernel-based Machine Learning. By using sparse matrix masking at the source level, OKRA not only ensures privacy under a semi-honest adversary model, but also achieves high computational efficiency.
%Our experiments, conducted across various clinical image datasets, evaluated model quality, computational performance, and resource overhead. The results showcase the performance, efficiency and scalability of OKRA.

%Arjhuns suggestion:
% In contemporary healthcare, the shift towards personalised medicine necessitates machine learning techniques that can effectively handle sensitive, high-dimensional medical image data distributed across various sources. This becomes critically important in the context of rare diseases, where limited data availability poses significant challenges to analysis. Addressing the critical need for privacy-preserving and computationally efficient methods, we introduce a novel geometric projection-based approach for kernel-based machine learning in a distributed environment. This technique, tailored for linear, polynomial, Gaussian and rational quadratic kernels, significantly enhances scalability and speed compared to current randomized encoding-based solutions. Our method demonstrates superior performance in securely and accurately computing kernel information, crucial for medical image analysis. Through comprehensive experiments, we establish our approach's efficacy in both privacy preservation and computational efficiency. 

%They offer robust and interpretable solutions, which is especially important in medicine. 
%Implementing Kernel methods becomes challenging, if the data sources are distributed and cannot be joined at a trusted third party for privacy reasons. 

%Medical imaging is key in modern medicine. From magnetic resonance imaging (MRI) to microscopic imaging for blood cell detection, diagnostic medical imaging reveals vital insights into patient health. To predict diseases or provide individualized therapies, machine learning techniques like kernel methods have been widely used. Nevertheless, there are multiple challenges for implementing kernel methods. Medical image data often originates from various hospitals and cannot be combined due to privacy concerns, and the high dimensionality of image data presents another significant obstacle. While randomised encoding offers a promising direction, existing methods often struggle with a trade-off between accuracy and efficiency.
%Addressing the need for efficient privacy-preserving methods on distributed image data, we introduce OKRA (Orthonormal K-fRAmes), a novel randomized encoding-based approach for kernel-based machine learning. This technique, tailored for widely used kernel functions, significantly enhances scalability and speed compared to current state-of-the-art solutions. Through experiments conducted on various clinical image datasets, we evaluated model quality, computational performance, and resource overhead. Additionally, our method outperforms comparable approaches. %The results showcase the performance, efficiency and scalability of OKRA.

% Removed some redundancies and mentioned rare diseases - 
Medical imaging, ranging from MRI to microscopic imaging, is crucial in modern medicine for revealing vital patient health insights. Kernel methods are widely used in machine learning to predict diseases and provide individualized therapies. However, implementing these methods faces challenges due to privacy concerns and the high dimensionality of image data, often sourced from various hospitals. Existing randomized encoding methods struggle with balancing accuracy and efficiency.
To address these issues, we introduce OKRA (Orthonormal K-fRAmes), a novel randomized encoding-based approach for kernel-based machine learning. OKRA, tailored for commonly used kernel functions, significantly improves scalability and speed over current state-of-the-art methods. Experiments on various clinical image datasets demonstrate our method's superior model quality, computational performance, and resource efficiency.


\end{abstract}
